EM-Paste: EM-guided Cut-Paste with DALL-E Augmentation for Image-level Weakly Supervised Instance Segmentation

We propose EM-PASTE: an Expectation Maximization(EM) guided Cut-Paste compositional dataset augmentation approach for weakly-supervised instance segmentation using only image-level supervision. The proposed method consists of three main components. The first component generates high-quality foreground object masks. To this end, an EM-like approach is proposed that iteratively refines an initial set of object mask proposals generated by a generic region proposal method. Next, in the second component, high-quality context-aware background images are generated using a text-to-image compositional synthesis method like DALL-E. Finally, the third component creates a large-scale pseudo-labeled instance segmentation training dataset by compositing the foreground object masks onto the original and generated background images. The proposed approach achieves state-of-the-art weakly-supervised instance segmentation results on both the PASCAL VOC 2012 and MS COCO datasets by using only image-level, weak label information. In particular, it outperforms the best baseline by +7.4 and +2.8 mAP0.50 on PASCAL and COCO, respectively. Further, the method provides a new solution to the long-tail weakly-supervised instance segmentation problem (when many classes may only have few training samples), by selectively augmenting under-represented classes.

==> sections/alg/extract.tex <==
\begin{algorithm}[H]
    \caption{Foreground Extraction}\label{alg:extract}
    \hspace*{\algorithmicindent}\textbf{Input:} Set of images $\mathcal{I}=\{I_i\}_{i=1}^N$, set of labels $\mathcal{Y}=\{\mathbf{y_i}\}_{i=1}^N$, image classifier $f(\cdot)$ with feature extractor $\phi(\cdot)$, class of interest $a$  \\
    \hspace*{\algorithmicindent}\textbf{Output:} Set of image foregrounds $\mathcal{O}=\{{O}_i\}_{i=1}^N$ of class $a$ objects.
\begin{algorithmic}[1]
    \LineComment Step 1: Region proposal
    \State $\mathcal{O} \gets \emptyset$
    \ForAll{image ${I}_i \in \mathcal{I}$ where $y_i^a=1$}
        \State $\mathcal{S}_i \gets \text{EntitySeg}(I_i)$
        \State $c_i^a \gets \textnormal{center of \gradcam}(I_i,a)$
        \State $p_s \gets f(s) \textnormal{ for top $n$ segments } s \in \mathcal{S}_i \textnormal{ with smallest } \text{dist}(s,c_i^a)$
        \State $\mathcal{O} \gets \mathcal{O} \cup \{\arg\max_s\{p_s\}\}$
    \EndFor
    \For{$j$ iterations}
        \Statex\hspace{\algorithmicindent}$\triangleright \textnormal{ Step 2 (Maximization):}$
        \State $r_{i} \gets \phi(O_i),\,\forall O_i \in \mathcal{O}$
        \State $\hat{m} \gets \textnormal{mean of } r=\{r_i\}_{i=1}^N$
        \State $\mathcal{O'} \gets \textnormal{k\% of } O_i \in \mathcal{O} \textnormal{ near } \hat{m}$
        \State $r'_i \gets \phi(O_i'),\, \forall O_i' \in \mathcal{O'}$
        \State $\hat{m}' \gets \textnormal{mean of } r'=\{r'_i\}_{i=1}^N$
        \LineComment Step 3 (Expectation):
        \State $\mathcal{O} \gets \emptyset$
        \ForAll{image $I_i \in \mathcal{I}$ where $y_i^a=1$}
            \State $\mathcal{S}_i \gets \text{EntitySeg}(I_i)$
            \State $sim_s \gets \text{sim}(\phi(s), \hat{m}'),\, \forall s \in \mathcal{S}_i$
            \State $\mathcal{O} \gets \mathcal{O} \cup \{\arg\min_s\{sim_s\}\}$
        \EndFor
    \EndFor
\end{algorithmic}
\end{algorithm}

==> sections/method.tex <==
Our proposed $\model$ (Extract-augment-paste) pipeline consists of three main steps: foreground extraction (\Cref{sec:Foreground Extraction}), background augmentation (\Cref{sec:aug}), and compositional paste (\Cref{sec:paste}). Here are the details:

\subsection{Foreground Extraction}
\label{sec:Foreground Extraction}
Mask refinement
Train a model and whole process is a interactive process.


Pipeline for select correct foreground given one class. EM match

Step 1
%
\begin{comment}
(1) given one class (ambulance), the foreground of the ambulance (N), we use entity segmentation method to turn each image as several segments. (N images X m segments).

(2) we use image label to get the gradcam for each image. (N images X 1 gradcam outputs)

(3) For each image and each class, we use the grad-cam as seed (describe the distribution of gradcam highlighted region as one Gaussian based on their x-y position, we have the center of the Gaussian.) (This center is determined by finding the moment of the gradcam highlighted region instead of Gaussian center which may diverge and fail in some cases)
% When there are multiple objects for same class, we 

(4) For each gradcam Gaussian(moment) center, we find the segment that has smallest pixel-wise average distance to the center. (select 1 form m segments for each Gaussian) (select k segments that have the shortest distances to center from m segments, then use the classifier to choose one segment with the highest probability, k may vary for different classes)
(On ImageNet, this matching step result into ~70\% accuracy, percentage of the correct foreground.)
For PASCAL VOC, this matching step result into ~50\% accuracy. 
\end{comment}

\VV{Let us use mathematical notations for terms, equations for center calculations or pixel-wise distance calculations.}
%
\VV{Let us start with the goal of this step.}
In this step, the goal is to first generate a set of candidate segments that can correspond to foreground object mask.
%
Given an input image, we use entity segmentation method to obtain a set of segments of the image. 
%
%Using the same image and a label of an object that is presented in the image as input of Grad-CAM, an activation map which only highlights the key region that is associated with the prediction is generated. 
In addition, given the ground truth object label, we also generate the GradCam activation map \cite{} for the image that is associated with the predicted label. 
%
We then calculate the x-y coordinate of the center of moment of the GradCam activation region. \VV{How do we calculate the center of moment? Can we write as equation?}
%
We ignore segments of the input image that might be potential noise or background (segments with small areas, large bounding box, etc.) \VV{What are the other criterion to ignore segments}. For each segment, we calculate a pixel-wise average distance to the GradCam actionmap region center. 
%
In this way, the segment that contains the center usually has the shortest average distance to the GradCam center and is most probable to be the foreground object. 
%
%However, in mane edge cases, for example, when there are multiple objects of the same class presented in the image, the center might be out of the highlighted region generated by Grad-CAM. To resolve this, we keep $n$ segments with the shortest distances to the center, and pass them through the same classifier used in Grad-CAM. The segment with the highest predicted probability is our initial selection of foreground of the input image.
%
We observe that this is generally true when there is only one object present in each image. 
%
But, in many images, more than one object from the same class can be present. In this case, the foreground object may not overlap with the GradCam activation map. 
%
To resolve this, we keep $n$ segments with the shortest distances to the center. We pass them through the same classifier used in Grad-CAM \VV{More description is needed here.}. The segment with the highest predicted probability is our initial selection of foreground of the input image.


Step 2 (Maximization)

\begin{comment}
(1)For each segment, we first use Corrosion Algorithm to remove the small artifacts, we paste the foregournd into a minimum bounding box and then resize it as (299x299) image and padding with gray pixel. Then we get the latent representation after a specific layer of the classifier, and then compute the mean for the latent encoding of the N foreground segments for each class. 

(2) keep k\% of the foreground that near the center of the cluster, to rule out the outliers. 

(3) Compute the new mean of k\% correct foreground in 2048-dim (Xception)
\end{comment}
\VV{Start with the goal of this step.}
In this step, we want to first obtain a representative mean of the latent space representations of the object class.
%
For each foreground segment selected in step 1, we first use an erosion algorithm \cite{} to remove small potential artifacts and noise pixels in the segment. Then, we paste the foreground segment onto a minimum bounding box resized to 299 by 299 with gray padding. 
%The latent space representations of the segments are obtained by passing each processed segment to the same classifier we used in Grad-CAM, and we extract the feature vector of the last convolution layer of the classifier network as its latent space representation. 
%
We then generate latent space representation of each segment by passing it through the classifier used in GradCam. In particular, we use the feature of the last convolution layer of the classifier as the latent representation for the segment.
%
A mean vector of latent space representations of all selected foreground segments is computed. Further, we rule out outliers by keeping $k\%$ of the segments that are closest to the mean based on (Euclidean distance/cosine similarity). Based on the remaining foreground (inlier) segments, we compute a new mean of the latent space representations.

Step 3 (Expectation)

\begin{comment}
(1) again get (N images X m segments).
for each image (m segments), we get the latent representation of each segments use the classifier. 
(2) Then we compute the (cosine similarity) of each segments to the mean of the class, and we selecet the segments has the highest cosine similarity as the foreground segement.
(percentage of the correct foreground >90\% )
We iterate Step 2 and Step 3. 
Bimodel, GMM, clustering.
\end{comment}
\VV{Let us again specify the purpose of this step.}
In this step, we want to regenerate the set of foreground segments by matching segments with the updated mean obtained from the Maximization step.
%
For all of the images, we extract a set of segments for each image again using the same entity segmentation method mentioned in step 1 and drop the ineligible segments, and then we extract their latent space representations using the classifier network again. \VV{This seems to be one time process. This step seems to be shared in Step 2 and Step 3.}
%
We then compute a cosine similarity between each latent space representation of the segment of the image and the new mean obtained from step 2. The segment with the highest cosine similarity is select as the new foreground of the image. With a new set of foreground segments, we can perform step 2 followed by step 3 again for several iterations.



\begin{figure}[htbp]
\center{
    \includegraphics[center,scale=0.45]{figures/step1.pdf}
    \caption{Step 1 of foreground extraction. (a) Entity Segmentation is used to extract segments from images. (b) Grad-CAM highlights a region based on the given label, and the center of moments (white dot on the image) is calculated for the highlighted region. (c) For all sufficiently large segments, we compute the pixel-wise average distance to the center of region highlighted by Grad-CAM. (d) For $n$ segments that have the shortest distances to the center, a predicted probability is obtained using the classifier network for each segments, and we select the segment with the highest probability as the foreground of the image. (e) All of the foreground segments are filtered again using the classifier network, and we keep the foregrounds with predicted probability higher than a preset threshold.}
}
\end{figure}

\begin{figure}[htbp]
\center{
    \includegraphics[center,scale=0.7]{figures/EM_update3.png}
    \caption{Step 2 and 3 of foreground extraction. (a) After erosion and resizing, each extracted foreground is passed to the classifier, and a latent representation of the image is extracted using a bottleneck layer. (b) Using the mean of all latent representation, we keep k\% representations that are close to the the mean and rule out outliers. (c) The mean is updated after ruling out the outliers. (d) For each image, latent representations of all eligible segments are obtained by the classifier network. (e) The segment with the highest cosine similarity to the updated mean is selected as the new foreground of the image. (f) After obtaining a new set of foregrounds, they are used as input of step 2 of the next iteration.}
}
\end{figure}


%%%%%%%%%%%
%%%%%%%%%%% Sec 3.2 background augmentation
%%%%%%%%%
\subsection{Background (Context) Augmentation} \label{sec:aug}
On all training images, we use image caption method to describe the image, and we put the caption as input to DALLE, and then get the synthesized background images from DALLE.


%%%%%%%%%%%
%%%%%%%%%%% Sec 3.3 Compositional Paste
%%%%%%%%%
\subsection{Compositional Paste} \label{sec:paste}
% Goal is creating a "balanced" augmented dataset.
Once we have a list of extracted and augmented \todo{check} foregrounds, we create synthetic dataset by pasting the foregrounds into images. Our proposed algorithm tries to utilize the remaining available  background region to the maximum. We describe in detail our paste method below, layout our algorithm in \Cref{alg:paste}, and give an illustrative example in \Cref{fig:paste}
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.33\linewidth}
        \caption{Original image to be pasted.}\label{fig:paste1}
        \includegraphics[width=\linewidth]{figures/paste1.png}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.33\linewidth}
        \caption{The \textcolor{red}{red circle} is the max inscribing circle found based on contour.}\label{fig:paste2}
        \includegraphics[width=\linewidth]{figures/paste2.png}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.33\linewidth}
        \caption{Pasted image.}\label{fig:paste3}
        \includegraphics[width=\linewidth]{figures/paste3.png}
    \end{subfigure}%
    \caption{Illustrative example of our paste algorithm in \Cref{alg:paste}. In this example, a person is pasted on the image of an aeroplane. In part (b) the max inscribing circle is found from contour based on region without aeroplane i.e. blue sky. Note that the person is scaled to match the size of the circle found in part (b), and a random rotation is performed.}
    \label{fig:paste}
\end{figure}

The input is a list of images paired with extracted foreground. We note that initially we only have one extracted foreground for each image. We iterate through all images in line \ref{alg:line:init_start}, and paste $n_p$ other extracted foregrounds into the iterating image $I_i$. 
First we randomly select $n_p$ from $\mathcal{I}$ based on pre-defined distribution $p$ in line \ref{alg:line:select}, which will be discussed $p$ latter \todo{leave to users to decide}. Then in line \ref{alg:line:contour}-\ref{alg:line:pastedone} we iteratively paste images from those selected $n_p$ images onto $I_i$ by finding the background region where no foreground lies in and pasting the new foreground in this region, with matching size. To be specific, we first find the maximum inscribing circle from contour of $I_i$, which is computed on the region that is not region occupied by any foreground objects in $\mathcal{F}_i$. Then we scale the new foreground to match the size of the radius of the maximum inscribing circle. Last we rotate the new foreground by a random degree and paste at the center of the max inscribing circle.

Our intuition is to force the pasted images to occupy as many region of the pasted background as possible,  while remaining non-overlapping between the new to-be-pasted foreground and existing background and already pasted foregrounds. The scaling makes sure that the empty region can be utilized fully, while random 2D rotating ensures the diversity of the pasted image. In addition, in line \ref{alg:line:pastedone} to paste the object onto $I_i$, we note that direct pasting might lead to unwanted artifacts, as shown in the findings of \citet{dwibedi2017cut} and \citet{ghiasi2021googlesimple}. To mitigate this issue, we apply a variety of blendings on each pasted image, including Poisson blurring, Gaussian blurring, no blending at all, or any combination of those. In practice, we find only Gaussian blurring alone can yield sufficiently strong performance. We implement \Cref{alg:paste} using \texttt{opencv} \cite{opencv_library}.

The pre-defined selection distribution $p$, used in line \ref{alg:line:select}, is important in that it imposes the class distribution of synthetic dataset produced by \Cref{alg:paste}. There are two type of $p$ we investigate in this work. The simplest type is uniform distribution, i.e. selecting each image in $\mathcal{I}$ with the same chance. With this choice, the synthetic data largely follows the class distribution of $\mathcal{I}$. The second type is balanced sampling, i.e. giving the classes with more instances a smaller weight to be selected while giving the classes with less instances a larger weight. This setting helps each class to appear in synthetic data in about the same quantity. In \Cref{sec:longtail} we show that this setting is beneficial for long tail problem.

The number of paste images $n_p$ is important in that a value too low results in sparse foregrounds, while a value too small results in crowded foregrounds, each of those hurts the model learning. We have tried the values of 2 and 4 and empirically find 4 is sufficiently better. 
We note that in principle we can run \Cref{alg:paste} multiple times and/or restrict the iteration in line \ref{alg:line:init_start} to generate synthetic data of any size. In all our experiments we generate around 20k pasted images as our synthetic training set.
